Multiple Pedestrians and Vehicles Tracking in Aerial Imagery: A Comprehensive Study

In this paper, we address various challenges in multi-pedestrian and vehicle tracking in high-resolution aerial imagery by intensive evaluation of a number of traditional and Deep Learning based Single- and Multi-Object Tracking methods. We also describe our proposed Deep Learning based Multi-Object Tracking method AerialMPTNet that fuses appearance, temporal, and graphical information using a Siamese Neural Network, a Long Short-Term Memory, and a Graph Convolutional Neural Network module for a more accurate and stable tracking. Moreover, we investigate the influence of the Squeeze-and-Excitation layers and Online Hard Example Mining on the performance of AerialMPTNet. To the best of our knowledge, we are the first in using these two for a regression-based Multi-Object Tracking. Additionally, we studied and compared the L1 and Huber loss functions. In our experiments, we extensively evaluate AerialMPTNet on three aerial Multi-Object Tracking datasets, namely AerialMPT and KIT AIS pedestrian and vehicle datasets. Qualitative and quantitative results show that AerialMPTNet outperforms all previous methods for the pedestrian datasets and achieves competitive results for the vehicle dataset. In addition, Long Short-Term Memory and Graph Convolutional Neural Network modules enhance the tracking performance. Moreover, using Squeeze-and-Excitation and Online Hard Example Mining significantly helps for some cases while degrades the results for other cases. In addition, according to the results, L1 yields better results with respect to Huber loss for most of the scenarios. The presented results provide a deep insight into challenges and opportunities of the aerial Multi-Object Tracking domain, paving the way for future research.

==> sections/archive.tex <==
\subsection{Computer Vision and Remote Sensing}
Computer vision and aerial imagery are related fields, both aiming at computer understanding of images. The goal of traditional computer vision is to make a computer autonomously perform some of the tasks the human visual system can perform and to infer something about the environment in which a picture was taken \cite{prince2012computer}. In contrast to pure image processing, the output of a computer vision algorithm gives back information about the given image, and not of a new picture. Information can be anything such as object detection and recognition results, camera position, 3D models, and image segmentation. Although computer vision tasks often seem trivial for humans, they remain highly complex for computers since visual perception is not bound to any specific environment, and since different types and amounts of occlusions can limit the view on a target. Additionally, a target can move, and hence,  can be seen from different views and with different lighting conditions \cite{szeliski2010computer}. Nevertheless, there has been much progress in the field, especially with the rise of machine learning and deep learning, the affordable and easy access to computing power and the availability of mobile technologies offering massive amounts of photo and video data. Recently, computers surpassed the reported human-level-performance on the ImageNet dataset~\cite{imagenet_cvpr09} for object classification \cite{he2015delving}.  Medical imaging, machine inspection, facial recognition, pattern detection, surveillance, motion capturing, and feature matching are other fields of application for computer vision~\cite{szeliski2010computer}. 

In contrast to computer vision, remote sensing deals with different scenarios such as observing the earth and the environment from space or very high altitudes and retrieving information from these observations. During the fast development of remote sensing, it provided us with a better understanding of weather and climate, leading to a more precise weather forecast, offers a cheap and effective way of collecting information of vast spatial regions, and provides methods to monitor ground objects over time~\cite{barrett2013introduction, remoteSensing2008}. Such information is useful to analyze the development of rural and urban areas or the evolution of agricultural processes by providing repetitive knowledge on crop status during different times of a season. These are only few examples. Others also include atmospheric research, data collection with different scales, resolutions, and sensors, analysis of ecological systems, mapping of wildfires and natural resources, and coordination of emergency responses \cite{remoteSensing2008, everaerts2008use}. In recent years, the development of better camera systems made very high-resolution image ground data available. The higher level of detail opened the field for new areas of application, especially for remote sensing tracking approaches dealing with small objects such as vehicles, ships, or pedestrians~\cite{reilly2010detection, meng2012object, bahmanyar2019multiple}. 

\subsection{Machine Learning}

This section gives an overview of machine learning and introduces deep learning. Machine learning pursues to provide knowledge to computers through data and observations, which allows the computer to generalize to new situations. Machine learning tasks are divided into three categories: supervised learning, unsupervised learning, and reinforcement learning \cite{dey2016machine}. 

In supervised learning, a function maps inputs to specific outputs. Such inputs are provided as datasets \(D = (x_1,x_2,..)\), where \(x_i\) can be almost any kind of data, such as images, video files, sound files, point clouds, or time-series data \cite{schmidhuber2015deep}. Each sample \(x_i\) is paired with a desired output value \(y_i\), which is called the ground truth. Afterwards, an algorithm can learn a function by analyzing the data and map unseen samples correctly. The ground truth can either be a discrete label or a continuous variable, dividing supervised learning into classification and regression tasks. Common datasets for classification are the MNIST dataset \cite{lecun-mnisthandwrittendigit-2010} containing handwritten digits, CIFAR-10 \cite{krizhevsky2009learning} which consists of more than 60,000 images for image classification as well as MS-COCO \cite{lin2014microsoft} containing images for object detection and segmentation. Popular regression datasets cover, for example, house price prediction given the details of houses and their neighborhood as well as predicting the quality of wine given specific attributes \cite{harrison1978hedonic, cortez2009modeling}.

The goal of unsupervised learning is to find previously unknown patterns or learn the underlying distribution of data given a dataset \(D = (x_1,x_2,..)\). In contrast to supervised learning, the samples \(x_i\) are not paired with an output value \(y_i\). Instead, unsupervised learning aims to cluster similar samples within the data, perform density estimation, or solve association problems, for example. 

Reinforcement learning mainly optimizes the actions of software agents in a given environment. The agent has no knowledge of which actions to take until it has been into a specific situation. Based on its own decisions, it receives a reward depending on the outcome of its action. Future decisions are affected by this reward. The final goal is to maximize the reward in order to maximize the agent's performance. 


This thesis includes approaches based on supervised learning and deep learning. Hence, we will deepen the basics of these in the next sections.


\subsubsection{Deep Learning \& Neural Networks}
A neural network is a computer system that can learn and perform task-specific jobs without being explicitly programmed \cite{goodfellow2016deep}. It consists of an input layer, one or multiple hidden layers, and an output layer. The input of such networks is a vector which is transformed by the hidden layers of the network. In each of these layers operate neurons, producing an output based on a received input. Initially, random weights are assigned to each connection between the neurons, and bias is assigned to each neuron. These weights and biases are updated during the training process of the network, leading to more accurate outputs. The overall process is called backpropagation \cite{hecht1992theory}. The term deep learning emerged as networks got more and more layers, and hence got "deeper". \autoref{fig:neuralnet} shows an example network with one hidden layer.

However, for computer vision tasks dealing with image or video data, networks based on such fully connected layers do not scale well. For example, a single neuron in the first hidden layer with an input image of size \(300 \times 300 \times 3\) (i.g. 300 width, 300 height, 3 color channels) has \(300 \times 300 \times 3 = 270,000\) weights. CNNs deal with this problem by using a combination of convolutional, pooling, and fully connected layers. Convolutional layers consist of \(k\) filters of different sizes \(W \times H\). The filters are slid across the input image and compute dot products between the entries in the filters and the entries in the input resulting in \(k\) 2D activation maps, which are stacked to obtain the output \cite{o2015introduction}. Pooling layers reduce the spatial size of the output to decrease the amount of computation and parameters in the network. Networks built upon such structures play a key role in this thesis.

\begin{figure}[htpb]
  \centering
  \includegraphics[width=0.45\textwidth]{figures/neural_net.jpeg}
  \caption[Neural network architecture.]{Neural network with hidden layers. Retrieved January 3, 2019: \url{http://cs231n.github.io/neural-networks-1/}} \label{fig:neuralnet}
\end{figure}


\subsubsection{Layer Types}
During the experiments of this thesis, we used various layer types. While explaining every type of layer in detail is beyond the scope of this thesis, we introduce unfamiliar ones in the following.

\subsubsubsection{Local Response Normalization}
\gls{lrn} layers are not-trainable. They perform a lateral inhibition by applying a squared normalization over an input with multiple channels. 

\begin{equation}
    b_c = a_c \Bigg( w + \frac{a}{n} \sum_{c'=max(0, c-n/2)}^{min(N-1, c+n/2)} a_{c'}^2 \Bigg) ^{-\beta}
\end{equation}
, where \(a_c\) and \(b_c\) are the channel values before and after normalization, respectively, \(w\) is a value to provide numeric stability, \(n\) is the amount of neighboring channels used for normalization, \(a\) is a normalization constant and \(\beta\) is the exponent.



\subsubsubsection{Squeeze-And-Excitation Layers}
CNNs extract image information by sliding spatial filters across the input on different layer levels. While lower layers extract information such as edges and basic shapes, higher layers can detect more advanced structures such as cars or text. Nevertheless, each filter has a different relevance concerning the final output of the network. Within any layer, the filter amount is equal to the output depth. However, every output channel is weighted equally. \gls{se} Layers  \cite{hu2018squeeze} change this behavior by weighting each channel adaptively while adding less than one percent of computing cost. Each channel is squeezed to a single value by using global average pooling  \cite{lin2013network}, resulting in a vector with \(k\) entries. This vector is given to a fully connected layer reducing the size of the output vector by a certain ratio, followed by a \gls{relu} activation function. The result is fed into a second fully connected layer scaling the vector back to its original size and applying a sigmoid activation afterwards. In a final step, the idea is to weight each channel of the original convolution block by multiplying the results of the SE block.

 

\subsubsection{Activation Functions}
The activation function calculates the output of a neuron based on its input. In order to make neural networks capable of approximating any arbitrary function, activation functions need to be non-linear functions \cite{cybenko1989approximation}. Since neural networks need to be optimized during the training process, activation functions also need to be monotonic and differentiable. Commonly used activation functions are the sigmoid function, the hyperbolic tangent, or \gls{relu}.

\begin{comment}
\begin{figure}
  \centering
  \includegraphics[width=0.7\textwidth]{figures/activations.jpg}
  \caption[Activation Functions.]{Activation Functions. Retrieved January 2, 2019: \url{https://towardsdatascience.com/complete-guide-of-activation-functions-34076e95d044}}
  \label{fig:activationFunctions}
\end{figure}
\end{comment}

Sigmoid and tangent are recently losing popularity since they both suffer from the vanishing gradient problem. ReLU solves the problem of vanishing gradients by using a linear function with the positive x-axis. Nevertheless, since the output of all negative values is zero, neurons can "die" once they have a negative value. In order to solve this issue, ReLU was extended by Leaky ReLU, which has a predefined negative slope and PReLU, which aims to learn the slope of the activation function \cite{maas2013rectifier, he2015delving}. Other activation functions include ELU, Maxout, and Swish, which was recently proposed by Google \cite{ramachandran2017swish}.  \autoref{fig:activationFunctions} shows the functions and the graphs of some of the mentioned functions.

\subsubsection{Loss Functions}
Loss functions measure how well neural networks model the given data. They compare the output of the network with the ground truth and calculate the cost or the error. The loss function optimizes the network's weights \textit{w} until an error threshold is met. It is also essential that the loss function is differentiable since neural networks update all parameters by applying backpropagation. This subsection introduces the losses relevant to this master thesis.




\subsubsection{L1 \& L2 Loss}
The L1\footnote{https://pytorch.org/docs/stable/\_modules/torch/nn/modules/loss.html\#L1Loss} and L2\footnote{https://pytorch.org/docs/stable/\_modules/torch/nn/modules/loss.html\#MSELoss} losses are useful when dealing with regression problems. The L1 loss measures the \gls{mae} between the output of the network \(x\) and the ground truth \(y\). It is calculated as followed:
\begin{equation}
    L1(x,y) = \sum_i|x_i-y_i|
\end{equation}

The L1 loss is less affected by outliers than the L2 loss. The L2 loss  calculates the error of the squared distance between the network output and the true value:

\begin{equation}
    L2(x,y) = \sum_i(x_i-y_i)^2
\end{equation}

\subsubsection{Huber Loss}

The Huber loss \cite{huber1992robust} is a mixture of the L1 and the L2 losses and combines their good properties. It is given as the \gls{mse} when the error is small and calculated as the \gls{mae} when the error is big.
\begin{equation}
    L_H(x,y) =  \sum_i z_i
\end{equation}
\begin{equation}
    z_i = \begin{cases}
0.5(x_i-y_i)^2, & \text{$if |x_i-y_i|<1 $}\\
|x_i-y_i|-0.5, & \text{$otherwise$}
\end{cases}
\end{equation}

The Huber loss is more robust to outliers than the L2 loss and improves the L1 loss regarding missing minima at the end of the training.


